SoK: Cross-Domain MEV

We examine the current state of the cross-domain world, with particular focus on the protocols being used/planned for use by multi-domain users. We build on existing frameworks for analyzing how MEV is extracted, while also adding a new categorization of intrinsic-extractable value vs. time-extractable value to describe how MEV is generated for an extractor. Together, this provides us with a framework with which we compare classes of protocols enabling cross-domain MEV, and the MEV occurring within these classes. We analyze each protocol class separately and compare current implementations to an ideal functionality for each. We primarily focus on analyzing the MEV mitigations that these protocols provide, both now, and into the future. In each case, we also outline the technical barriers that current protocol implementations face. With this methodology, we identify sequencers and order-flow auctions as cross-domain protocols with the greatest potential to mitigate MEV, but also as protocols with some of the biggest technical barriers.

==> ACMSubmissionData.tex <==

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
	



\copyrightyear{2023}
\acmYear{2023}
\setcopyright{rightsretained}
\acmConference[DeFi '23]{Defi 23}{November, 2023}{Denmark}
\acmBooktitle{DeFi '23}
\acmPrice{}
\acmDOI{10.1145/1}
\acmISBN{1/22/11}

\settopmatter{printacmref=true}


==> BlogPost.tex <==
\section{By Hook or by Crook: Cross-Domain MEV Retention in Uniswap V4}

\textit{This research is funded by the Uniswap Foundation}

The long-anticipated release of Uniswap V4 is upon us. This blog post sketches a straightforward combination of a singleton pool and hooks within the new V4 framework to tackles cross-domain MEV at the source: the block producer. 

I'd been doing a couple of months of research on cross-domain MEV sources within the DEX ecosystem, and it almost always came back to the same term: Loss-versus-rebalancing or LVR. LVR put a name to the face of one of the primary costs incurred by DEX liquidity providers. Block builders on any chain are being goose-stepped into profit maximizing machines. To do this requires a knowledge of the most recent state of the primary exchanges and market-places, such as centralized exchanges and other large blockchains, not to mention the swaps in the mempool. The first, \textbf{guaranteed} cost that a DEX must pay is that of arbitraging the DEX's stale reserves to line up with the block builders best guess of where the underlying price is. From here, the builder then sequences the DEX swaps in a way so as to maximize the builders back-running profits. This proceeding sequence of back-runs pays fees to the pool, but are not guaranteed to take place.

It is only the arbitrage of the pool reserves that is guaranteed. This can be addressed with some hooks. 


The exact implementation of hooks hasn't been nailed down yet, but in this article we assume, as in the whitepaper (LINK), that a hook implements custom logic before or after 4 key phases in the pool contract:
\begin{enumerate}
    \item Initialize: When the pool is deployed
    \item Modify Position: Add or remove liquidity.
    \item Swap: Execute a swap from one token to another in the V4 ecosystem.
    \item Donate: Donate liquidity to a V4 pool. 
\end{enumerate}

\subsection{The Solution} 

Our proposed solution is based on similar techniques as used in \cite{DiamondMcMenamin}. We are only interested in hooks before and after swaps. For a particular pool, we make a distinction between the first swap interacting with the pool in a block, let's call this $\texttt{swap}_1$, and all other swaps, which we denote $\texttt{swap}_2$. For our solutions we introduce an LVR rebate function $\beta: \{1,...,Z \} \rightarrow [0,1]$. It suffices to consider $\beta()$ as a strictly decreasing function with $\beta(Z)=0$, for some $Z \in \mathbb{N}$. Whenever we call a hook, let $B_\text{current}$ be the current block number when the hook is called, and $B_\text{previous}$ be the number of the block in which the most recent swap occurred. We also need to introduce the idea of a vault contract \texttt{vault}, and a hedging contract $\texttt{hedger}$. 

Depositing $x_A$ token $A$s to \texttt{hedger} increases a contract variable \texttt{hedgeAvailableA} by $x_A$ (likewise \texttt{hedgeAvailableB} for token B deposits).  At all times, the block builder can submit a transaction removing some amount of tokens $x_A$ from \texttt{hedger} if at the end of the transaction $\texttt{hedgeAvailableA}>x_A$. If the builder withdraws $x_A$ tokens, reduce  $\texttt{hedgeAvailableA} $ by $ x_A$.



\subsection{Solution}

In this solution, consider the following logic(described algorithically as \texttt{beforeSwap()} and \texttt{afterSwap()} hooks in Algorithms 1, 2, and 3):


\begin{itemize}
    \item \textbf{If} $B_\text{current}-B_\text{previous}>0$, the swap is $\texttt{swap}_1$. Send  any remaining tokens in \texttt{hedger} to pool. After this, add some percentage of the tokens in \texttt{vault} back into the pool.\footnote{The correct percentage is the subject of further research.} Set the \texttt{hedgeAvailable} variables to 0.

    Execute $1-\beta(B_\text{current}-B_\text{previous})$ of $\texttt{swap}_1$, and remove the required amount of token $A$ from the pool so the implied price of the pool is equal to the implied price given $\texttt{swap}_1$ was executed. This is necessary because if only $1-\beta(B_\text{current}-B_\text{previous})$ of $\texttt{swap}_1$ is executed the price of the pool will not be adjust to reflect the information of $\texttt{swap}_1$. Add the removed tokens to $vault$.

    \item \textbf{Else}, it must be that $B_\text{current}-B_\text{previous}==0$, which implies the swap is a $\texttt{swap}_2$. Let $\texttt{swap}_2$ be buying some quantity $x_A$ of token $A$. One of the following three conditions must hold:
    \begin{itemize}
    \item \textbf{If }$\texttt{hedgeAvailableA}\geq x_A $ AND $x_A>0$, then execute $\texttt{swap}_2$ and decrease \texttt{hedgeAvailableA} by $x_A$, but do not remove any tokens from \texttt{hedger}. Increase \texttt{hedgeAvailableB} by $x_B$.

    \item \textbf{Else if }$\texttt{hedgeAvailableB}\geq x_B $ AND $x_B>0$, then execute $\texttt{swap}_2$ and decrease \texttt{hedgeAvailableB} by $x_B$, but do not remove any tokens from \texttt{hedger}. Increase \texttt{hedgeAvailableA} by $x_A$.

    \item \textbf{Else} there is not enough tokens deposited to perform the swap, then revert. \end{itemize}
\end{itemize}








\subsection{What does this solution solve?}

This solution allows the producer to move the price of the block to any level with $\text{swap}_1$, although only executing $1-\beta(B_\text{current}-B_\text{previous})$ of $\text{swap}_1$. This $\text{swap}_1$ can be thought of as the LVR swap, and is such it is discounted. From there, the producer is forced to match buy orders with sell orders. Orders are only executed against the pool if they can also be executed against the tokens in the hedge contract \texttt{hedger}. If the price does not return to the price set after $\text{swap}_1$ (the tokens in \texttt{hedger} don't match the \texttt{hedgeAvailable} variables,) there are sufficient tokens in \texttt{hedger} to rebalance the pool, and these tokens in the hedging contract are used to do so in the next block the pool is accessed. 

An ideal solution would allow the producer to execute arbitrary transactions, and then repay $\beta$ of the implied swap between the start and end of the block, as this is seen as the true LVR (the end of block price is the no-arbitrage price vs. external markets, otherwise the producer has ignored a profitable arbitrage opportunity). Our solution does this in a roundabout way, although using hooks. The producer moves the price of the block to the no-arbitrage price in the first swap, and is then forced to return the price here at the end of the block, all through hooks. 

\subsection{Does the solution work?}

\vspace{0.2cm}
\begin{center} \texttt{yes} \end{center}

\vspace{0.2cm}

How? This solution differs from the theoretical proposal of \cite{DiamondMcMenamin} in 2 important functional ways. Firstly, \cite{DiamondMcMenamin} depends on the existence of a censorship-resistant auction to convert some \% of the vault tokens so the vault tokens can be re-added into the liquidity pool. The solution provided above directly readds the vault tokens into the pool. Through simulation, we have identified the solution provided in this document approximates the returns of the protocol in \cite{DiamondMcMenamin} and its perfect auction when the amount being re-added to the pool is less than 5\% per block. 


Don´t just take our word for it! The simplest solution of \cite{DiamondMcMenamin} periodically re-adds the retained LVR proceeds from the vault into the pool at the pool price. We include the graph of the payoff of this protection applied to Uniswap V2 pool vs. a Uniswap V2 pool without this protection. The payoff of this protocol is presented in Figure \ref{fig:PerfectRetention}. The expected returns of the protected pool relative to the unprotected over 180 days (simulated 1,000 times) is 1.057961. This is almost exactly equal to the derived cost from \cite{LVRRoughgarden} of 3.125bps per day:
\begin{equation}
    \frac{1}{(1-0.0003125)^{180}} \approx 1.05787.
\end{equation}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{Images/PCA100pctRetention.png}
    \label{fig:PerfectRetention}
\end{figure}

Unfortunately, 100\% LVR retention is unrealistic. Let's instead assume an average LVR retention of 75\% (An LVR rebate parameter of 0.75). Through simulation, the \cite{DiamondMcMenamin} protocol-protected UniV2 gives a relative return vs the unprotected UniV2 of 1.0431. The relative returns of the protocol described in Algorithm \ref{alg:ReAddAlgo} applied to UniV2 vs unprotected UniV2 are plotted in Figure \ref{fig:ReAddcomparison} for several re-add percentages (amount of the vault to re-added to the pool each block). The average relative returns are 1.0456, 1.0436, and 1.0335, for re-add percentages of 1\%, 5\%, and 12.5\% respectively. 


\begin{figure}
    \centering
    \includegraphics[scale=0.45]{Images/ReAddPercentages.png}
    \label{fig:ReAddcomparison}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{Images/HODL.png}
    \label{fig:HODLcomparison}
\end{figure}

From this, we can see that the 1\% re-add strategy each block actually \textit{outperforms} the optimal conversion strategy. This is because for simulations with large moves, converting the pool is less profitable (HODLing is the optimal in these scenarios). If we introduce fees related to pool size, we can counteract this out-performance. In Figure \ref{fig:HODLcomparison}. we include a representation of the performance of the theoretical conversion protocol of \cite{DiamondMcMenamin}, our re-adding protocol, and HODLing, all vs. the corresponding unprotected UniV2 pool.

\subsection{Casting the Hooks Wider}
    
Based on the typical limit-order model for Uniswap, the above implementation might seem highly restrictive for user orders. One way that we can improve UX and likelihood of execution is by allowing users to be price-agnostic, incentivizing market orders. When we hear about market orders.



\begin{algorithm}[H]
\def\baselinestretch{1} \scriptsize \raggedright
\caption{Low Impact Re-Adding}\label{alg:ReAddAlgo}
	\begin{algorithmic}[1]
	    
        \State \texttt{address hedger, vault}
        \State \texttt{uint} $B_\text{previous}$ \Comment{Block where previous swap occurred}
        \State \texttt{mapping beta()} \Comment{an implementation of a strictly decreasing function over the range [0,1]}
        \State \texttt{float truePrice}

    
        \SPACE
        
	\Hook{\texttt{beforeSwap(int $x_A$, int $x_B$)}}{} \Comment{A swap of $x_A$ tokens for $x_B$ tokens}
		\If{$B_\text{current}-B_\text{previous}>0$} \Comment{True for first swap in block}
                \State \texttt{hedger.drain()} \Comment{Reset hedging contract}
                \State \texttt{vault.reAdd()} \Comment{Add some \% of vault tokens to pool}
                \State \texttt{swapDiscount=1-$\texttt{beta}(B_\text{current}-B_\text{previous})$} \Comment{Discount applied to $1^{st}$ swap every block}
                \State \texttt{truePrice=simulateSwap($x_A$, $x_B$).price() }\Comment{ `true price' if full swap was executed}
                \State \texttt{swap(swapDiscount*$x_A$,swapDiscount*$x_B$)} \Comment{swap with discount applied}
                

            \Else \Comment{The swap is not the first swap this block}
                \If{$\texttt{hedgeAvailableA} \geq x_A \textbf{ AND } x_A>0$} \Comment{Swap is attested \& buying token A}
                    \State \texttt{swap($x_A$, $x_B$)}
                \ElsIf{$\texttt{hedgeAvailableB} \geq x_B \textbf{ AND } x_B>0$} \Comment{Swap is attested \& buying token B}
                    \State \texttt{swap($x_A$, $x_B$)}  
                \Else \Comment{It must be $\texttt{hedgeAvailableB}<x_B$ AND $\texttt{hedgeAvailableA}<x_A$}
                    \State \texttt{revert()} \Comment{Price is not attested}
                \EndIf
            \EndIf
        \EndHook

        \SPACE
        
        \Hook{\texttt{afterSwap()}}{} 
		\If{$B_\text{current}-B_\text{previous}>0$} \Comment{True for first swap in block}
                \State \texttt{vault.rebalance(truePrice)} \Comment{Ensure pool price==truePrice}
                \State \texttt{$B_\text{previous}=B_\text{current}$} \Comment{If statement will return False for rest of block}

            \Else \Comment{The swap is not the first swap this block}
                \If{$\texttt{hedgeAvailableA} \geq x_A \textbf{ AND } x_A>0$} 
                    \State \texttt{hedger.hedgeAvailableA-=$x_A$} \Comment{Reduce token A attestation budget}
                    \State \texttt{hedger.hedgeAvailableB+=$x_B$} \Comment{Increase token B attestation budget}
                    

                \ElsIf{$\texttt{hedgeAvailableB} \geq x_B \textbf{ AND } x_B>0$} 
                    \State \texttt{hedger.hedgeAvailableB-=$x_B$} \Comment{Reduce token B attestation budget}
                    \State \texttt{hedger.hedgeAvailableA+=$x_A$} \Comment{Increase token A attestation budget}
                \EndIf
            \EndIf
        \EndHook

	\end{algorithmic} 
	
\end{algorithm}

\begin{algorithm}[H]
\def\baselinestretch{1} \scriptsize \raggedright
\caption{Hedger}
	\begin{algorithmic}[1]
	    
        

        \State \texttt{address owner} \Comment{Tracks current player executing orders (probably block builder)}

        \State \texttt{uint hedgeAvailableA, hedgeAvailableB} \Comment{Tokens (`budget') that pool can sell from current state}


        \State \texttt{address V4Pool, vault}

        \SPACE
        
        \Function{\texttt{deposit()}}{}
            \State \texttt{hedgeAvailableA+= deposited token As}
            \State \texttt{hedgeAvailableB+= deposited token Bs}
            \State \texttt{owner=msg.sender}
        \EndFunction

        \SPACE
        

        \Function{\texttt{withdraw(withdrawA, withdrawB)}}{}
            \State \texttt{require hedgeAvailableA, hedgeAvailableB  $\geq$ withdrawA, withdrawB} 
            
            \State \texttt{transfer withdrawA, withdrawB from this contract to msg.sender}
            \State \texttt{require hedgeAvailableA, hedgeAvailableB -= withdrawA, withdrawB} 
        \EndFunction

        \SPACE
        
       \Function{\texttt{drain() onlyV4Pool}}{}
            \State \texttt{transfer all tokens from this contract to pool}
            \State \texttt{hedgeAvailableA, hedgeAvailableB=0}
        \EndFunction
	\end{algorithmic} 
	
\end{algorithm}

\begin{algorithm}[H]
\def\baselinestretch{1} \scriptsize \raggedright
\caption{Vault}
	\begin{algorithmic}[1]

        \State \texttt{address V4Pool}
        
        \State \texttt{float pctToReAdd}
        \State \texttt{uint minimumTokenA\_ToReAdd}  \Comment{A fixed value. Ensures vault eventually empties}
        \State \texttt{uint minimumTokenB\_ToReAdd}  \Comment{A fixed value. Ensures vault eventually empties}
        
        \SPACE
        
        \Function{\texttt{reAdd() onlyV4Pool}}{} \Comment{Re-Adds tokens from vault to pool}
            \State \texttt{transfer max(pctToReAdd*tokenA\_Balance, minimumTokenA\_ToReAdd)  to V4Pool}

            \State \texttt{transfer max(pctToReAdd*tokenB\_Balance, minimumTokenB\_ToReAdd) to V4Pool}
        \EndFunction

        \SPACE
        
        \Function{\texttt{rebalance(truePrice) onlyV4Pool}}{} \Comment{Sends pool tokens to vault (LVR Retention)}
            \State \texttt{remove tokens from pool and send to vault so pool.price()=truePrice} \Comment{The tokens removed are always the tokens being bought}
        \EndFunction
        
	\end{algorithmic} 
	
\end{algorithm}




==> BlogPost2.tex <==
\section{It's not Ehm-ee-vee, it's miss-ee-vee}

When trying to address MEV, there are many approaches. Initially, we identified protocols where MEV occurred and proposed improvements which on average reduced the costs being incurred by users. This was iterated until we reached something we were happy with, or we identified maxima that protocol design on its own could not solve. 

As in medicine, the first solution for a disease is treatment, but the end-goal is a cure. To find a cure, we need to know the source. 

This article proposes a perhaps not-so-new categorization of MEV sources as either as a result of mis-pricing or mis-timing. Mis-pricing is relatively straightforward as a concept. If a contract or transaction is mis-priced, a builder can instantaneously act on the state/resulting state in the case of a transaction, and extract value from it. Mis-pricing can be extended to include sub-optimal social welfare maximization. Although an important source of value being lost (some would argue the most important), it is not value being extracted. Research must be devoted to welfare maximization, although it is important to distinguish social welfare maximization, the maximum net utility that can be gained by a set of players in a given time-frame/interaction, and MEV, value that is being taken from one player by another. We neither want maximal welfare with maximal MEV nor minimal MEV with minimal welfare. 

Mis-timing is more complex, and covers a variety of time-based value that is either gained or lost. Contracts and transactions are exposed to the time-value they give up between revealing the state (last block update for a contract, time of transaction submission in the case of a transaction) and when the state can be acted on. In this time, all other participants in theory (in reality only the proposer and builders) can wait until the instant before the state can be updated to decide on what action to take on the state. 

Mis-timing goes deeper, and darker. Typically, there is no obligation that a contract or transaction state needs to be acted on. As such, mis-timing can be induced, and exacerbated, by proposers. Another word for this is censorship. While a contract or transaction is being censored, there is some cost being incurred by the contract or transaction in question. In the case of a contract, if users cannot access the contract state, the contract has less value to those users, who may then take their business, fees, and network effect, to name but a few value propositions, to a competitor. If a proposer is collaborating with the competitor, this value is being extracted. In the case of a transaction, consider an auction where censoring a player trying to submit a higher bid than you, results in a substantially lower clearing price. Value extracted. 

==> DeFi/DeFiMain.tex <==
\section{Introduction}



The reality of a multi-domain world is fast approaching, and it may already be upon us. To compete for MEV, there is an ever-increasing need for value extractors to exist on as many blockchains and domains as possible, even co-locating with block proposers. While this is not necessarily a bad thing if there is a high degree of competition and decentralization, this game is typically winner takes all \cite{FlashboysOG}, which is definitely a bad thing.
Previous work in the space has tried to define cross-domain MEV \cite{obadia2021unity} and hypothesize about how MEV changes in a cross-domain world. Despite the formalism in that work, it is unclear how to apply the provided formal definitions to draw qualitative or quantitative conclusions about cross-domain MEV. We note that \cite{obadia2021unity} is a self-proclaimed work-in-progress, and is likely intended to be thought-provoking rather than a standard for reasoning about cross-domain MEV in blockchain protocols. 

We present a systematization of prominent cross-domain protocols focusing on the types of MEV that occur within each protocol. To do this, in each of the protocols, we breakdown the MEV occurring there by how the value is extracted, and where the value originates for the extractor. These categorizations are described in detail in Sections \ref{sec:how} and \ref{sec:whereFrom} respectively. By using a consistent set of distinguishing factors to describe the MEV occurring in cross-domain protocols, we allow for a clearer understanding of the MEV that is occurring in these protocols, and what protections these protocols provide, both now and into the future. As many of the most promising cross-domain protocols are still in the early stages of development, we also discuss the barriers that these protocols face.

Our analysis identifies the censorship-resistant ideal functionalities of shared sequencers (Section \ref{sec:sequencers}), multiple single-domain sequencers (Section \ref{sec:multisequencers}), and batch settlement protocols (Section \ref{sec:Batch} as viable solutions to cross-domain MEV, and MEV in general.\footnote{Off-chain requests for quotes/interactions (RFQs) also have the potential to mitigate MEV. As RFQ protocols require liveness from both users and LPs, and our analysis in Section \ref{sec:where} tries to compare the effect of the introduced protocols on extractable value in automated market makers, we include discussions on off-chains RFQ protocols in Appendix \ref{sec:RFQs}. It is possible that RFQs emerge that allow for passive LPs, as in AMMs.} All of these protocols are not without technical barriers, as described in the respective sections, but stand as areas of particular interest for further research. 

\section{Cross-Domain MEV $\subseteq$ MEV}\label{sec:Categories}



There are many potential categorizations for, and components of, MEV. We can consider extractable value based on how the value is extracted (Section \ref{sec:how}), where the value originates (Section \ref{sec:whereFrom}), who controls access the extractable value \cite{3EV}, where the extraction occurs, how the extracted value can be isolated (e.g. proposer-builder separation (PBS, see Appendix \ref{sec:PBS}), order-flow auctions (see Section \ref{sec:OFAs}), etc.), who the extracted value can be redistributed to (users vs. builders vs protocols vs. everyone), to name but a few. 
In this work, we focus on the initial two areas; how the MEV is extracted and where the extractable value is originating. Using these categories and components, we provide insight into the cross-domain MEV landscape, especially within the protocols that we introduce in Section \ref{sec:where}. 

We consider extractable value from the extractor's perspective. We note that extractor value may vary depending on ability to propose blocks, capital, latency, etc.. We generalize the notion of extractor to be the extractor with the most value to gain, as this is typically the extractor that wins the right to perform the extraction (at least in the PBS model). Furthermore, extractor value vs. user/protocol value is not necessarily zero-sum, because of the utility that users and protocols get from performing blockchain actions, making the sum of utilities positive. Most of the time however, extractor value gained is user/protocol value lost. 

\subsection{How Value is Extracted}\label{sec:how}

This categorization has already been developed through a series of blog-posts advocating it \cite{FrontierSignalvsOrdering}. To summarize, MEV is either extracted as a result of \textit{ordering} or \textit{signal}. Extraction due to ordering involves strategically inserting and sequencing a set of transactions to be executed, where the value of tokens at the start of the sequence is greater than the value at the end of the sequence, using on-chain data only. The clearest example of this is starting the sequence with some token $X$, and ending the sequence with a greater balance of token $X$, although it can be extended to tokens with the same peg (although this has its limitations \cite{USTDepeg,USDCDepeg}). Ordering extraction was popularized in the original Flashbots paper \cite{FlashBoys2.0} (signal extraction was not), and quantified here \cite{FlashbotsExploreWebsite}.

Signal extraction is based on information occurring off-chain which creates a profitable opportunity to submit a set of transactions on-chain. Signals can occur in the mempool, on other blockchains, centralized exchanges, in news headlines, to name but a few. A signal-based extractable value opportunity occurs when the value to act on some transaction or on-chain state for an extractor becomes higher as a result of new off-chain information. 
With a knowledge of underlying token valuations and/or the existence of hedging opportunities off-chain, signal opportunities involve the extractor starting and ending the on-chain extraction sequence in different tokens. It is with these valuations/off-chain opportunities that the starting token balance is worth less than the final balance to the extractor.

A common example of signal extraction is loss-versus-rebalancing \cite{LVRRoughgarden}, when the price of a token swap on a centralized exchange moves sufficiently far away from an on-chain AMM price, creating a profitable opportunity for an extractor to realign the AMM with the centralized exchange price. 

Both of these extraction techniques are used in blockchains. The profit from ordering for extractors, after paying for the right to extract, is almost 0 due to its risk-free nature (fork attacks aside) and its deterministic valuation (approximately the same profit for all extractors). Profit from signal extraction is much more subjective, depending on factors like risk-appetite, access and costs to trade against centralized exchanges, signal latency, etc. 


\subsection{Where the Extractable Value Originates}\label{sec:whereFrom}




This categorization has likely been hinted at in other works, although we have not seen it explicitly used. We propose that the expected extractable value of a transaction can be be split into mutually exclusive \textit{intrinsic-extractable value} and \textit{time-extractable value} components. This is exactly the same way options are valued \cite{OptionsPricing}. We note that due to extractor competition, the time at which positive extractable value opportunities can be acted on typically corresponds to the time at which the extractable value opportunity must be acted on. There are exceptions to this, particularly related to monopolization of inclusion/censorship powers. In what follows, we assume that the first time at which a state/transaction creates a positive extractable value opportunity corresponds to time when the state/transaction must be acted upon. We refer to this time as \textit{expiry/expiration}.\footnote{When censorship is possible, time-extractable value is bounded below by time-extractable value between now and the first time at which the state can be acted on.  However, expected-extractable value can decrease between state-update times (e.g. decreasing variations of the fee escalators introduced here\cite{FeeEscalator}).} 

\begin{itemize}
    \item \textbf{Intrinsic-extractable value} is the expected value to the extractor at the time when the blockchain state or transaction must be acted on.
    For a Uniswap order, this can be approximated by the maximum of the expected value of all of the front-running and back-running opportunities. For a Uniswap pool, it is the expected extractable value from moving the price up or down at the instant when orders are to be included in the blockchain (typically arbitraging the price in line with all other on- and off-chain liquidity).  Intrinsic-extractable value can be realized when the time to act on the order of blockchain state is 0 (the order/state must be acted on now). 
    \item \textbf{Time-extractable value} is slightly more complex. With respect to a blockchain protocol/transaction state on which the extractor can act on, the time-extractable value can be derived in a similar way to that of an option. The extractor has the length of time between confirmation times/blocks to decide whether or not to act on the blockchain state in question. The time-extractable value to the extractor of this optionality is the sum of all paths with a positive extractable value at expiration, times the probability of that path happening. \\
    For user transactions, time-extractable value is similar. For a transaction, the time value to an extractor is the expected value that can be extracted from the transaction between seeing the transaction and including the transaction. This is again analogous to options pricing. Examples of time-extractable value are provided in Appendix \ref{sec:Examples}.
\end{itemize}



\subsubsection{Using Intrinsic- vs. Time-Extractable Value to Analyze MEV}


When examining the MEV occurring in each of the protocols in the proceeding section, we consider the effects that these protocols have on both intrinsic- and time-extractable value. Intrinsic-extractable value can be reduced by things like batch execution, reduced slippage requirements, and encrypting some or all a transaction's data. Reducing time-extractable value is simpler in theory: reduce the time extractors have to act on a state, the time until expiration. As we will see in the proceeding section, this is fraught with complications. Another way to reduce the net time-extractable value paid by a user or protocol is charging for the time-extractable value that protocols and users give up (see Section \ref{sec:priority}), as is done in options trading.
For the purpose of this document, it suffices to understand that the time-extractable value for a protocol/transaction grows with respect to time until expiration, as in Figure \ref{fig:TimeValue}. As the time with which extractors have to act on a protocol or transaction approaches 0, so too does the time-extractable value, collapsing to the intrinsic-extractable value. 


\section{Cross-Domain Protocols and MEV}\label{sec:where}


\begin{table}
\scalebox{0.52}{
\begin{tabular}{|l|c|c|c||c|c|||c|c||c|c|}
    \toprule
     & &  \multicolumn{4}{|c|}{\textbf{Current Implementations}} & \multicolumn{4}{|c|}{\textbf{Ideal Functionality}}  \\
    \midrule
     & & \multicolumn{2}{|c|}{\textbf{Origin}} & \multicolumn{2}{|c|}{\textbf{How Extracted}} & \multicolumn{2}{|c|}{\textbf{Origin}} & \multicolumn{2}{|c|}{\textbf{How Extracted}} \\
    \midrule
    \textbf{Protocol} & \textbf{Sec.} & \textbf{Intrinsic} &\textbf{Time} & \textbf{Ordering} &\textbf{Signal}&\textbf{Intrinsic} &\textbf{Time} &\textbf{Ordering} & \textbf{Signal} \\
    \midrule
    Multi-domain Sequencers & \ref{sec:sequencers} & \userMaybe \ \LPMaybe & \userMaybe \ \LPMaybe & \userMaybe \ \LPMaybe & \userMaybe \ \LPMaybe & \userNo \ \LPNo & \userNo \ \LPNo & \userNo \ \LPNo & \userNo \ \LPNo \\
    \midrule
    Single-domain Sequencers & \ref{sec:multisequencers} & \userMaybe \ \LPMaybe & \userMaybe \ \LPMaybe & \userMaybe \ \LPMaybe & \userMaybe \ \LPMaybe & \userNo \ \LPNo & \userNo \ \LPNo & \userNo \ \LPNo & \userNo \ \LPNo \\
    \midrule
    Order-flow auctions  & \ref{sec:OFAs} & \userMaybe \ \LPYes & \userMaybe \ \LPYes & \userMaybe \ \LPYes & \userMaybe \ \LPYes & \userNo \ \LPYes & \userNo \ \LPYes & \userNo \ \LPYes & \userNo \ \LPYes \\
    \midrule
    App-chains & \ref{sec:AppChains} & \userYes \ \LPYes & \userYes \ \LPYes & \userMaybe \ \LPMaybe & \userYes \ \LPYes  &  \userNo \ \LPNo & \userYes \ \LPYes &  \userNo \ \LPNo & \userYes \ \LPYes \\
    \midrule
    Priority Auction & \ref{sec:priority} & \userYes \ \LPMaybe & \userYes \ \LPMaybe & \userYes \ \LPMaybe & \userYes \ \LPMaybe & \userYes \ \LPNo & \userYes \ \LPNo & \userYes \ \LPNo & \userYes \ \LPNo \\
    \midrule
    Batch Settlement & \ref{sec:Batch} & \userYes \ \LPYes & \userYes \ \LPYes & \userMaybe \ \LPMaybe & \userYes \ \LPYes &  \userNo \ \LPNo  &  \userNo \ \LPNo  &  \userNo \ \LPNo  &  \userNo \ \LPNo  \\
    \midrule
    Encrypted Mempool & \ref{sec:encrypted} & \userMaybe \ \LPYes & \userMaybe \ \LPYes & \userMaybe \ \LPYes & \userMaybe \ \LPYes &  \userNo \ \LPYes &  \userNo \ \LPYes &  \userNo \ \LPYes &  \userNo \ \LPYes \\
    \midrule
    Slot Auctions & \ref{sec:slots} & \userYes \ \LPYes  & \userYes \ \LPYes  & \userYes \ \LPYes & \userYes \ \LPYes  & \userYes \ \LPYes & \userYes \ \LPYes & \userYes \ \LPYes &  \userYes \ \LPYes  \\
    \midrule
    Reduced Block Times & \ref{sec:reducedBlockTimes} & \userYes \ \LPYes & \userYes \ \LPYes & \userYes \ \LPYes & \userYes \ \LPYes & \userYes \ \LPYes &  \userNo \ \LPNo & \userYes \ \LPYes &  \userNo \ \LPNo \\
    \bottomrule
  \end{tabular}} 
   \caption{A breakdown of extractable value for users and LPs withing an AMM, when order submission to the AMM is controlled by the respective cross-domain protocols.\label{table:RelatedWorkComparison} The following labels* indicate the corresponding MEV component: \\
  \userNo/\LPNo :\ is effectively eliminated in the corresponding protocol for users/LPs. \\
  \userYes/\LPYes :\ exists in the corresponding best-in-class protocol for users/LPs.\\
  \userMaybe/\LPMaybe :\ is theoretically eliminated for users/LPs, but current implementations have seen limited deployment, depend on centralized trust, or significant technical barriers remain.\\
   *\footnotesize{Readers should consult the respective subsections for full details on the extent of these indicative labels, and the assumptions made related to the ideal functionalities.}}
   \vspace{-0.9cm}
\end{table}
 


This section introduces a list of protocols at the core of cross-domain conversation. All of these protocols play some role in cross-domain MEV, with some protocols explicitly intended to provide some sort of MEV mitigation. In each of the protocols we discuss both the type of value extraction taking place (Section \ref{sec:how}), and where the extractable value typically originates (Section \ref{sec:whereFrom}). With each protocol we describe the ideal protocol functionality, current implementations, and open questions that exist towards implementing the ideal functionality specified. We also describe the state of MEV in each, including, but not limited to, cross-domain MEV.  As this area of research is still in the early stages, Appendix \ref{sec:moreProtocols} extends our analysis to other protocols being considered as cross-domain MEV solutions. Protocols in this extended analysis may emerge as more viable contenders in the future.



We consider the centralization of power at any point in the transaction/block-building/MEV supply-chain, whether relaying, building, running an auction, or block proposing, as negative for protocols. If protocols centralize power to a small set of players, strict rules and incentives must be in place to ensure these players behave correctly. These rules and incentives do not exist as a given, and require careful construction.  In-keeping with the core decentralization values of blockchains,  we highlight centralizing effects that protocols have. Furthermore, in each such protocol, we leave the ``Can the protocol protect against such effects?'' as an important open question.


\subsection{Framework for Analysis}

We consider blockchains as state machines. Blockchains can be represented as a directed acyclic graph, with each block containing state machine updates. The updates in a block $B$ act on the state achieved by applying all blocks in the directed sub-graph reachable from $B$. Where multiple competing sub-graphs exist, blockchain protocols have tie-breaking rules for deciding which sub-graph to choose (most blocks, greatest height, etc.). Unless otherwise stated, blocks contain a sequence of transactions (state machine updates) which must be applied in order, with this sequence chosen by a single elected block proposer for each block\footnote{Protocols can force (see Sections \ref{sec:sequencers} and \ref{sec:multisequencers}) or incentivize (see Section \ref{sec:slots} and Appendix \ref{sec:PBS}) proposers to our-source sequencing.}. Blocks are added to the blockchain at discrete time intervals.

Where appropriate, our analysis focuses on the MEV occurring in an AMM where order submission is controlled by the respective protocols. We isolate the MEV being extracted from the users submitting orders for inclusion, and liquidity providers (LPs) deploying liquidity, in the AMM pools. A summary of this analysis is provided in Table \ref{table:RelatedWorkComparison}.



 


\subsection{Shared Sequencer}\label{sec:sequencers}

\subsubsection{Ideal Functionality}

A single entity, the shared sequencer, accepts transactions for 2 or more blockchains, committing to include valid transactions in the order in which they are sequenced. Commitments can take place at any time (independently to block production time on the sequenced chains). The validity condition for transactions can range from fee payment, at a minimum, to `the transaction is executable in the given sequence'.

In an ideal implementation of a shared sequencer, the delay between valid transaction submission from users, and inclusion in the sequence of transactions is negligible. Furthermore, all builders are incentivized to obey the shared sequencer (for this to be true, builders would need to face economic punishment for disobeying the shared sequencer), and there is some way for builders to charge and control fees in the shared sequencer.
Moreover, an ideal shared sequencer allows for atomic cross-chain transactions, which are discussed in Appendix \ref{sec:atomictxs}. 

All of this practically removes extractable value opportunities. Intrinsic extractable value is prevented as no processing of transactions is possible, removing an extractor's ability to strategically bundle transactions. Time-extractable value is effectively eliminated as a result of the negligible confirmation times for transactions, which means no time for extractors to wait for more profitable opportunities. As soon as an extractable value opportunity exists with respect to a protocol, an extractor must take it, or miss the opportunity. 

Shared sequencing is intended to shift at least some of the signal MEV extraction to ordering MEV extraction (signals that previously existed across domains would exist on the same domain in the shared sequencer). If sequencing is first-come first-served, ordering MEV would be removed. As time-extractable value approaches 0, so too does the profitability of signal MEV. 

\subsubsection{Implementations and Discussion}

Prominent shared sequencer implementations include Espresso \cite{Espresso}, Astria \cite{Astria}, and Zenith \cite{Zenith}. Detailed write-ups on Espresso, Astria, and shared sequencers in general can be found here \cite{CharbonneauSequencers1,CharbonneauSequencers2}. All of these implementations are currently focused on sequencing layer-2s.

 

\subsubsection{Open Questions}


Unfortunately, shared sequencers are highly complex and depend on strong assumptions that are unlikely to hold without significant technological and incentivization advancements. Specifically, there is currently no protocol to guarantee that proposers and builders on sequenced chains obey the sequencer. This may be related to the difficulties in provably ensuring availability of data for all sequenced domains. Without proof that a sequence of transactions was delivered, punishments for not adhering to the sequence are limited. Data availability proofs on Celestia \cite{Celestia}, a leading data availability protocol, take upwards of 10 seconds, slower than almost all block production times. In the PBS paradigm that exists in Ethereum Proof-of-stake, relayers collect built block information, and are responsible for providing that information to the proposer and validators when a block is selected for inclusion. If proposers on sequenced chains must build blocks according to sequencer restrictions, the entire sequence needs to be available to the proposer before blocks are built. 

Related to centralization of power, the end-game for shared sequencers may be to also build the blocks for sequenced domains, much in the same way as proposed in SUAVE \cite{SUAVEIntro}(discussed in Section \ref{sec:OFAs}). This potentially shifts all of the MEV/transaction fee revenue control to the shared-sequencer, which does not align with the current paradigm of proposers on the individual chains controlling this revenue. 
A rational sequencer who can induce even small sequencing delays can extract all of the intrinsic extractable value from transactions. With centralization of the sequencer, such attack vectors are likely possible and undetectable. That said, time-extractable value is likely to be negligible in any sequencer implementation.

Existing shared sequencer solutions do not require transaction validity checks, which is problematic for an shared sequencer.  If transactions are all-or-nothing, rational/malicious players may try to front-run one or more of the domains (on the shared sequencer) to invalidate the transaction. This in turn may invalidate all proceeding transactions in that domain. For a single domain where all-or-nothing restrictions are enforced naturally, this is not an issue.

There likely needs to be pre-processing or post-processing on shared sequencer transactions before the block is confirmed in which sequenced transactions are promised to be executable by one or more watchtowers. Incorrect (in)validation by a watchtower could then carry a severe penalty. These watchtowers can be executors or simply state-update checkers. There is a natural requirement therein to validate these transactions in the order they are sequenced. Although this is centralizing, a decentralized sequencer who can enforce punishments on these watchtowers neutralizes the bad effects it has (although if the validation is done before sequencing, we need competition. As such, post-processing is preferred, and can be done by even a single player, although we then need DOS protection).


\subsection{Multiple Single-Domain Sequencers}\label{sec:multisequencers}


\subsubsection{Ideal Functionality}

Each blockchain runs a sequencer, who commits to including valid sequenced transactions as they are sequenced. As in shared sequencers, this validity condition can range from fee payment, to executability. The delay between valid transaction submission from users, and inclusion in the sequence of transaction is negligible, with builders incentivized to obey the sequencer (for this to be true, builders would need to face economic punishment for disobeying the shared sequencer), and there is some way for builders to charge and control fees in the shared sequencer. Extractable value is eradicated in this ideal functionality, for the same reasons as the ideal functionality of the shared sequencer. Single-domain sequencers would not affect the signals existing outside of the chain being sequenced, although the signal MEV opportunities would reduce in line with the reduction in time-extractable value. 

\subsubsection{Implementations and Discussion}

A single-domain sequencer is exactly that; a sequencer in charge of a single blockchain. Arbitrum \cite{ArbitrumSequencer} and zkSync Era \cite{zksyncSequencer} are examples of blockchains using dedicated single-domain sequencers.
We have seen that shared-sequencer implementations are fraught with unsolved issues and considerations. In the short term, it seems we would be happier to accept the benefits of sequencing in a single domain at the expense of this added functionality. 

Furthermore, for a given transaction to be split across multiple domains, with single-domain sequencers, we can practically achieve much of the same functionality given the existence of cross-domain agents. Actions/intents requiring multiple domains can have conditional execution constraints controlled by the user, or delegated cross-domain executors.
As users can interact with directly with these cross-domain agents, the trust required is significantly less (pairwise economic/social/legal contracts can be established).

\subsubsection{Open Questions}

Current implementations of single-domain sequencers are centralized. Decentralizing the sequencer without degrading performance and usability is an active area of research. 
However, single-domain sequencers have significantly less technical barriers than shared sequencers, with connectivity and the alignment of incentives simplified in the single domain case. The trade-off here is the ability to execute cross-domain transactions atomically. As discussed above, this may not be such a big barrier.



\subsection{Order-flow Auctions}\label{sec:OFAs}


\subsubsection{Ideal Functionality}

Users are able to auction their orders/order information among a set of searchers. The proceeds of these auctions are returned to the user. An ideal cross-domain order-flow auction eliminates both intrinsic and time-extractable value for the user, assuming the order-flow auctions are indeed revenue maximizing. The revenue from such an auction should equal to total extractable value for the extractor.

Protocol-level value extraction (against the LPs) still remains. Multi-domain order flow auctions (like the proposed SUAVE protocol) will shift some of the signal MEV to ordering MEV in a similar fashion to shared sequencers.


The heavyweight contender in this domain is the Flashbots-proposed SUAVE (Single Unified Auction for Value Expression) chain \cite{SUAVEIntro}. Here, users can post transactions/intents to be executed across potentially many domains participating in the SUAVE domain. The general idea is for searchers (executors in the SUAVE notation) to compete via an auction to execute these intents, with some or all of the proceeds from this competition capturable by the user. The competition among searchers in SUAVE is intended to be based on partially encrypted transactions, with \textit{hints} provided by users revealing enough information to searchers to optimally bundle transactions, while retaining some form of pre-execution privacy, and the value that comes with it (extractable value that is not given to the searchers).

Searchers bundle transactions for inclusion in the SUAVE chain. The SUAVE chain logic then selects and orders the bundles maximizing the (extractable) value of the set of bundles according to the encoded valuation functions of the chain. These sets of bundles represent blocks to be added to participating blockchains. With enough participation, SUAVE is intended to act as a one-stop-shop for transaction submission across many blockchains. 

Uniswap have announced UniswapX \cite{UniswapXIntro}, an order-flow auction (Dutch Auction) to assist with routing in the proposed Uniswap V4 \cite{UniV4Release}. Due to the potential for thousands of liquidity pools for the same token pair in Uniswap V4, some off-chain routing is likely needed to ensure users receive the best possible pricing. Emulating a Dutch Auction among searchers to fill user orders should help in this regard. However, the UniswapX proposal also mentions the ability for auction winners to use their own private inventory/other on-chain liquidity, which might have negative implications for on-chain LP providers. A legacy order-flow auction protocol that appears to have shutdown in recent months is Rook \cite{RookWebsite}. 

\subsubsection{Open Questions}


SUAVE depends on a centralized auctioneer \cite{SUAVEUpdate} (Flashbots or an additional trusted third party). The Flashbots hope is that this auctioneer can eventually be replicated by some form of trusted execution environment, and eventually a transparent decentralized system. The path to such an end-goal remains unsolved and a contentious point. Trust in a trusted auctioneer appears to be widely accepted, at least in the case of Flashbots as the trusted auctioneer, evidenced by the amount of blocks produced by MEV-boost \cite{MEVBoostpct}, which also depends on trusting Flashbots as an auctioneer.

The removal of extractable value through revenue-maximizing off-chain auctions depends on many factors, including searcher competition and auctioneer trust, both of which need further investigation. 
Without atomicity guarantees, most searchers in these domains must charge fees to off-set the cost and probability of not executing intended orders on dependent domains. Specifically, if a searcher agrees to sell some amount of tokens to a user in the order-flow auction with the intention of/assuming that they will be buying those tokens back on Ethereum, the searcher must increase their fee proportionally to the cost of not executing the swap on Ethereum. Sequencers would practically eliminate this cost. With such costs, searcher competition likely diminishes, reintroducing extractable value opportunities for dominant searchers.

The logic around maximizing extractable value through re-ordering bundles is intended to be run by trusted execution environments \cite{MillerSUAVETEE}, such as trusted off-chain hardware or cloud infrastructure.
Centralizing power off-chain to trusted execution environments requires significant further study, with guarantees/limitations of such solutions clearly stated for the community. Another concern for order-flow auctions is the ability to auction bundles of orders in a revenue-maximizing way for users generating the orders. The concern here is the creation of incentives to spam the auction and fill bundles with fake orders, paying less revenue to the affected users. This is discussed in detail here \cite{mazorra2023optimal}.

With respect to UniswapX, questions remain about the effect that improved user execution has for on-chain LPs. Given a particular Uniswap V4 pool is trading with a user, this pool must be offering a better price than any other on- or off-chain liquidity source, which also means the LP's price is likely mis-priced. To this end, some defragmentation of liquidity (restrict the execution of orders to Uniswap pools only) might be required to remove this potentially toxic element of efficient routing through off-chain auctions. 

\subsection{App-Chains}\label{sec:AppChains}

\subsubsection{Ideal Functionality}

A single instance of the protocol is implemented on a dedicated blockchain, with users required to bridge their assets to and from the chain. App-chains likely eliminate the intrinsic extractable value of orders, but their effect on time-extractable value is not clear. Like previous protocols merging users/order-flow from multiple domains, app-chains will also shift some of the MEV from signal to ordering, although signal opportunities likely still remain in the discrete block time, single proposer model. Based on the thesis of Osmosis \cite{Osmosis}, ordering extractable will be fully redistributable to both users and LPs. 

\subsubsection{Implementations and Discussion}

Related to shared sequencers is the idea of app-chains. An app-chain is exactly that, a separate blockchain/side-chain on which all app-specific actions are carried out. For a protocol such as Uniswap with fragmented liquidity, isolated/unused domains are exposed to increased time-extractable value, in addition to the reduced fees from not being actively used. An app-chain removes this inter-protocol staleness. An app-chain remains exposed to $t$-staleness where $t$ is the time between confirmations on the chain. For a protocol like Uniswap, the hope would be the app-chain would adapt to the core needs of the protocol, and favour short confirmation times to address the costs associated with time-extractable value. 
App-chains also have the potential to reduce intrinsic-extractable value existing in the 1 app per chain paradigm by defragmenting liquidity, and the reduced slippage/higher indicative price accuracy this would bring. 

Examples of app-chains include Osmosis \cite{Osmosis}, dydx \cite{dydx}, and ThorChain \cite{ThorChain}. A detailed discussion on the value proposition of app-chains is provided here \cite{VariantAppChains}. 

An interesting feature of Osmosis, one of the emerging app-chains in the DEX space, is their prospective ProtoRev feature \cite{OsmosisProtoRev}. ProtoRev effectively tries to realign all on-chain liquidity sources after each transaction, back-running every transaction with an attempted arbitrage of on-chain liquidity pools against each other. The surplus from this process (there can only be a surplus under current conditions) is shared among the DAO controlling the Osmosis chain. 
Arbitrary post-processing is not considered plausible in general purpose L1 chains, due to the added computational cost. That being said, ProtoRev demonstrates the power that app-chains have given an ability to tailor consensus and execution specifically to the needs of the dedicated application. 

\subsubsection{Open Questions}


The main problem that app-chains face is the need to bridge assets to and from the app-chain (which may have prohibitive costs, including additional order staleness, depending on the bridge), and worse user experience as a result. App-chains on their own do not necessarily affect the timing issues that exist on normal blockchains. Therefore, it is important to understand the timing, trust and security specifications of any proposed app-chain when considering its use. 
It has been demonstrated that app-chains can potentially provide meaningful ordering protections where multi-purpose blockchains cannot \cite{ChitraUncertainty}. This is in line with the promises of Osmosis. The extent to which these protections can be provided for each application stands as an open question. 


\subsection{Priority Auction to Interact with Application First} \label{sec:priority}


\subsubsection{Ideal Functionality}

The ability to interact with the protocol is auctioned off, with proceeds paid to the protocol. This eliminates extractable value against LPs in expectancy, with the proceeds of both LP- and user-extractable value paid to the protocol itself. By explicitly capturing some of the MEV proceeds through the auction, net profitability is reduced, however, the gross MEV from ordering and signal techniques should remain largely unchanged.

\subsubsection{Implementations and Discussion}

A proposed implementation of this is MEV-capturing AMMs (McAMMs) \cite{McAMMs}, which proposes the protocol itself auctioning off the right to send the first swap to an Mc-AMM ahead of time, with reduced protocol performance if the transaction is not included. The auction proceeds should reflect the expected extractable value to be extracted from the pool within the block, both from the intrinsic extractable value of user orders, and the time-extractable value of both orders and the pool pricing function between blocks. In this regard, McAMMs have many similarities to slot auctions, although here the proceeds are more clearly exploited by the protocols themselves. 

Diamond \cite{DiamondMcMenamin}, a variation of a priority auction which shifts this auction to the builders, has both been described as a prospective Uniswap V4 pool \cite{DiamondV4}, following the release of Uniswap V4 specifications \cite{UniV4Release}. Builders must repay some percentage of the net tokens removed in the pool within the block. The final pool price in a block is claimed to correspond to the builders best guess of the true underlying price of the pool, with this net amount of tokens removed corresponding to the MEV as a result of time-value extraction. 
Comparing these two solutions, Diamond does not restrict access to any individual ahead of block production time, removing any possibility of denial-of-service attacks either on, or by, the player with the exclusive right to execute the first swap.  

\subsubsection{Open Questions}

Both of these solutions effectively require the builder/searchers to arbitrage the pool against this true price, and then provide liquidity to the user orders. In these solutions, the pool reserves play a limited role beyond providing users with an estimate of how their orders will be executed. On the other hand, the end game in PBS also appears to be for builders to implicitly provide liquidity to user orders, taking on inventory risk in order to extract all available value from a block. Importantly, McAMMs and Diamond return the value to where it is being extracted, as opposed to the block proposers in PBS, so has clear advantages over existing solutions in this regard.

Priority auctions likely incentivize private order-flow. By ensuring a significant share of order-flow, an extractor can better price priority auctions, allowing such an extractor to minimally increment the second best auction bid, guaranteeing priority. This creates a cycle, attracting more private flow. This in turn allows the extractor to provide private order-flow extracting arbitrarily high rents as the only player in town with access to the protocols offering priority. Such negative centralizing externalities need to be properly addressed.

Additionally, in the case where auctions must be carried out by a trusted auctioneer, such as in McAMMs, it is not clear if the incentives of the auctioneer are aligned with that of protocol. A clear specification and analysis of the role of the auctioneer is required.  



\subsection{Batch Auctions/Batch Settlement}\label{sec:Batch}

\subsubsection{Ideal Functionality}

Orders are executed at a common price. In an ideal functionality with no censorship, extractable value opportunities are effectively eliminated. 

\subsubsection{Implementations and Discussion}

The most common example of such a batch settlement protocol is CowSwap \cite{CoWSwapWebsite}. In CowSwap, orders are exposed to time-extractable value due to the previously discussed power of inclusion that solvers in the protocol have when deciding which orders to execute in a batch. It can be argued that intrinsic value is reduced, especially when some trust exists in the solvers, as orders are less likely to be maximally extracted against in a batch.  Penumbra \cite{Penumbra} also proposes batch settlement, with orders there encrypted, mitigating extractable value. In Penumbra, trust is placed in the threshold-decryption committee to not decrypt information prior to inclusion in the batch. 

\subsubsection{Open Questions}

Transaction censorship in batch auctions diminishes the benefits of such protocols, exposing users orders to both intrinsic- and time-extractable value. Furthermore, searchers and/or block producers in charge of order inclusion can estimate the imbalance of an auction, either from unencrypted order information or from the implicit information leakage through identity-reveal, timing, etc.. These players can then use their 'last-look' capabilities to enter an auction if the implicit settlement price of a batch is profitable. This is time-extractable value, albeit diluted amongst orders in a batch. Such value can be seen as a combination of both ordering and signal MEV, although we consider it more of a signal opportunity. How to reduce trust/censorship capabilities of searcher/solvers in current batch protocols is an important open question. 


\subsection{Encrypted Mempool}\label{sec:encrypted}


\subsubsection{Ideal Functionality}

Orders are committed to the blockchain before order information is revealed to the block producer. Orders are decrypted and executed at some point in the future. User-level extractable value is removed when no information about a user's transaction can be learned before it is executed. The effect on LP MEV is unclear. Although we would expect protocols to adjust to an encrypted mempool paradigm, in isolation (without batch execution for example) LPs remain exposed to value-extraction attacks, such as losses-versus-rebalancing. 

\subsubsection{Implementations and Discussion}

Secret Network \cite{SecretNetwork}, Osmosis \cite{Osmosis},  and Penumbra \cite{Penumbra} are examples of protocols using encrypted mempools. For detailed discussions on the effects of encrypted mempools on MEV see \cite{EncryptedMempoolsQuintus,EncryptedMempoolsCharb}.

\subsubsection{Open Questions}

As mentioned previously, trust is currently placed in decryption committees not to decrypt transactions before committing transactions to the chain. Solutions without a committee \cite{DelayEncryptionBurdges} are promising, although significant work is still required to make these techniques feasible at scale.
When generic state updates are encrypted, their executability and computational requirements are not necessarily known. This leads solutions like Penumbra and Osmosis to restrict the action space of transactions. Implementing encrypted mempools outside of application-specific chains like the ones mentioned remains an area requiring further research. 




\section{Conclusion}\label{sec:conclusion}

We provide a summary of cross-domain protocols, not only as a guide to understanding cross-domain MEV, but also as a resource for understanding the cross-domain world in general. Some of the most promising protocols for enabling a cross-domain world, such as shared sequencers and generalized order-flow auctions, are also the protocols with the most open questions. This highlights that the cross-domain world of today is still under construction, and will likely be very different to that of the future. This future will be shaped by the answers to the open questions that we have posed among others. As value is created in the cross-domain world, so to will value extraction opportunities. That being said, many of the ideal protocol functionalities of Section \ref{sec:where} effectively eliminate MEV, or allow for its redistribution.
Censorship and centralization are common barriers for many of the protocols that we discuss. These stand as areas that warrant particular focus from the research community. 

==> Discussion.tex <==
\section{Discussion}


\subsection{Trade-Offs}

Some of the solutions in the previous section aim to provide transaction atomicity. This is an instinctively desirable property, both from the user experience perspective, but also in reducing staleness of transactions. However, it must be made clear that no true solution exists in this regard. Synchronizing and providing exclusive to two or more domains, required for atomicity, also comes at a cost to the builder(s) providing this service. 


\begin{table*}
\scalebox{0.7}{
  \begin{tabular}{llll}
    \toprule
    Proposal & Advantages & Disadvantages & Trade-offs\\
    \midrule
    Shared Sequencer & Approaches Guarantees of CEX & Complex, must be at least as secure as participating domains & \\
    Sequencer for each domain & & & \\
    
  \end{tabular}}
  \caption[Comparison of Proposed Cross-Domain MEV Solutions]{.}
  
\end{table*}


==> Introduction/OurContribution.tex <==
\subsection{Our Contribution}

We present a systemization of literature on cross-domain value extraction. 


==> MeetingPrep.tex <==
\section{Meeting Notes}


Hey man! Enjoyed lunch, thanks again. 
Other possible cross-chain only use cases
 \begin{enumerate}
     \item Using fees/escrow on one chain to allow for a transaction on another. 
 \end{enumerate}

==> Prelims/Prelims.tex <==
\section{Preliminaries}


According to \cite{Zamyatin2019Communication} cross Chain communication is \textbf{impossible} without a TTP. This paper also does a good job at formalization of cross-chain messaging. 
\subsection{Shared Sequencers}



==> RelatedWork.tex <==
\section{Related Work}

The primary work in this area is the Unity vs. Strength paper \cite{obadia2021unity}. Since then, there has been a relative explosion in interest in the value being generated across domain. Whether due to the limitations of blockchain inter-operability \cite{berg2022empirical,Zamyatin2019Communication}, or something else, the extractable value in this space is believe to be largely unchanged (REFs). 


\subsection{Protocols Enabling Cross-chain Swaps}


ODOS, WooFi, HOP, DODO, Thorchain, Chainge all appear to offer cross-chain DEX solutions. Techniques include active MMs/ "solvers" who are incentivized to execute transactions on both chains. In the case of Thorchain, all assets are bridged to the chain, where swaps take place, and are then sent to the required chains.   An pseudo-academic solution, again involving oracles has also been discussed\footnote{\url{https://ethresear.ch/t/privacy-enabled-cross-chain-automated-market-maker/13115}}. 

\subsection{Cross-Domain Value Analysis}

Frontier \footnote{\url{https://frontier.tech/a-new-game-in-town}}, Mekatech \footnote{\url{https://meka.tech/writing/analysing-cross-chain-arbitrage-opportunities-for-atom-fee57867-4385-4ead-b19c-8db75a753226}}, Roughgarden et al. \cite{LVRRoughgarden}, all provide estimates for the amount of extractable value that exists between domains. The seeming best cross-chain arbitrage tracker is provided by ODOS \footnote{\url{https://www.odos.xyz/arbitrage}}, visualizing the paths to perform cross domain arbitrage

==> Sources.tex <==
\section{Understanding Cross-Domain MEV}

There are an increasing number of categorizations out there regarding MEV in general, whether by who can extract it (3EV REF) or where it is generated. The 3EV characterization feels rather complete: MEV can be extracted by privatizing access to information (Mafia), access to extraction (Monarch) or by co-ordination (Moloch. In the original 3EV characterization, this type of MEV is largely un-captured due to a lack of coordination). Ideally, protocols should be aware of which MEV prevails in its protocol. With respect to a DEX, all three are in effect. Mafia and Monarch are applicable to both the users sending orders, and the LPs providing liquidity. Moloch also negatively affects both users and LPs.
If Uniswap implementations across all chains were to be in constant communication, LVR would be greatly reduced. Due to the isolated nature of chains, this is not necessarily solvable. Similarly, if users were able to access all Uniswap liquidity across all chains when sending an order, execution prices would be strictly better (excluding fees).

\begin{definition}
    A domain is a state-machine, with each state-transition in the domain controlled by a set of rules. Domains are defined by a tuple $(T,\Delta)$, where $T$ is the minimum time between transitions, and for $\epsilon$ the expected time after the domain receives a valid transition proposal that the transition is applied to the domain, $\epsilon=\mathcal{O}(\Delta)$.
\end{definition}

\begin{example}
    CEXs are effectively (0,0)-domains. Under this definition, a censorship-resistant blockchain with blocks every $t$ seconds is a $(t,t)$-domain. As such, we can define censorship-resistant domains just by their minimum time between transitions
\end{example}

Now let us consider what this means for information dispersal across domain, and cross-domain transactions.

For CR domains $D_1,..., D_n$ defined by $t_1,...,t_n$, information from Domain $D_i$ can be applied to domain $D_j$ in time $\mathcal{O}(t_i+t_j)$. This is an upper-bound, and there are several important exceptions.

Letting $D_1$ be a CEX with the player in charge of applying transitions to $D_i$ having direct access to $D_1$, information from $D_i$ can be applied to domain $D_j$ in time $\mathcal{O}(t_j)$. This can be seen as any information to be applied to $D_i$ is immediately applied to $D_1$, which in turn can be applied $D_j$. In reality, fees on $D_1$ might prevent this information from being applied to $D_1$. In such a scenario, the information must be applied to $D_i$ first, resulting in $\mathcal{O}(t_i+t_j)$ to be applicable to $D_j$.

If the player controlling $D_i$ also controls $D_j$, information from transitions to be applied to $D_i$ can be applied to $D_j$ in time $\mathcal{O}(t_j)$. Furthermore, if the transition being proposed to $D_i$ is sent by a player who can send a transition proposal to $D_j$, the information can be applied to $D_j$ in time $\mathcal{O}(t_j)$. 

We now draw some parallels between the above scenarios and blockchains. For a professional trader trying to maximize their profits across all domains (REF), informational disadvantages leads to mis-pricing and sub-optimal profits. Most professionals have access to high-volume CEXs, although just listening to CEX information omits the information that does not get passed to CEXs, specifically information that is not actionable on the CEX, either because it falls within the fee bounds of the CEX, or because the player with the information is not able to interact with a CEX. Both of these vectors are highly centralizing, especially with growing regulatory scrutiny around CEXs (and the reduced liquidity/higher implicit fee this entails). Players are thus incentivized to control as many domains as possible. With the proposer-builder separation paradigm firmly in play, it is the block-builders that are receiving the transition proposals. Private order-flow has a stark effect in this paradigm, giving builders massive advantages, not only in building their own blocks, but in all blocks across all domains.  


For transactions that need to be executed in series across $k$ domains $D_a,...,D_k$, the time to execute the series is $\mathcal{O}(t_a+...+t_k)$.

To reason about the cross-domain world 

For the purpose of this article I will focus on a simplified categorization of how MEV occurs: Mis-pricedness vs. Staleness. There are other potential sources, such as censoring-related ransoms



\begin{definition}
    A state is \textit{well-priced} if a rational block-builder is indifferent to acting instantaneously on the state or not.
\end{definition}

\begin{definition}
    A state is mis-priced if a rational block-builder is incentivized to instantaneously act on the state.
\end{definition}

Without restrictions on what transactions a block-builder can include in a block, rational block-builders only include transactions if they are incentivized to do so. If someone sends a transaction to a builder, it is only guaranteed to be included instantaneously if it is mis-priced. This goes for contracts too, whether being deployed or updated. 

\begin{definition}
    A state is \textit{stale} if it is not acted on instantaneously. 
\end{definition}

With this high-level definition of staleness, every state in the blockchain ecosystem is stale. The important thing to note is staleness can be quantified. 

\begin{definition}
    A state is \textit{t-stale} if it has not been acted on in $t$ seconds. 
\end{definition}

This slightly more refined definition allows us to capture some important sources of MEV. As demonstrated in \cite{LVRRoughgarden}, if prices change with some expected distribution (volatility), we can estimate the cost that staleness has for LPs in AMM protocols. It is important to note that this cost is also incurred for user transactions. While transactions rest in the mempool, although the may have been well-priced at creation, they then leak MEV through staleness. The realized cost of $t-$staleness for a specific transaction or contract depends on the information that is revealed between the last update/creation and $t$.  

\begin{definition}
    A state is \textit{censored} if access to the state is being denied by a player or players in the system. 
\end{definition}


In addition to value being extracted from a state through staleness and mis-pricing, value can also be extracted by censorship. Protocols may have decreasing utility over time/between updates. If updates can be affected by a third-party, such as a block producer, the utility of a protocol can be reduced, causing players to pivot to alternatives. Examples include competing DEXs, protocols depending on oracle updates for access. If the third-party is invested in an alternative protocol, there is an incentive to delay these updates. 

In some ways, censorship is an example of induced staleness. 

\subsection{Mis-pricedness and Staleness in the Cross-Domain Space}

As the number of domains increases, mis-pricing increases, at least in expectancy. Each domain has unique information sources that take time to disseminate to all other domains. If there is a player who is able to see every domain's prospective state updates (transactions to be confirmed) at all times, this player is then capable of generating well-priced states that are not stale. Contrarily, users generating DEX transactions for a particular domain are almost guaranteed to mis-price transactions. This is purely due to a lack of visibility of all states. 

Although we typically expect block builders to instantaneously update centralized exchanges when they receive new/actionable/well-priced information, many builders might not have access to the main CEXs, while fees may prohibit such updates. Such builders might take on risk themselves within their own source domain, with other domains only seeing the information when the new information from the source domain.

With multiple domains, the best-case staleness for any individual domain is the best-case staleness of the domain itself: waiting for the next block on that domain. Multiple domains fragment the action space, and introduce bridging times/multi-domain confirmation times, and oracle response times. While users or contracts in a certain domain wait for signals from other domains, there is an inherent cost being incurred. If a user must wait for assets to be bridged before an order can be executed, builders may choose to omit the bridge transaction until the order becomes valuable due to staleness. If an AMM depends on an oracle to adjust price/fees, builders may omit such an update to benefit from the staleness of existing prices/fees. 

With information being processed out-of-domain before being applied to the domain (such as builders do to maximize MEV in a given block), staleness has a significant effect on MEV. The greater the staleness, the greater the expected cost for users and contracts \cite{LVRRoughgarden}. With more time for things to happen that affect the value of the state, more things will happen, in expectancy. As such, the cross-domain ecosystem, despite its benefits, increases both the expected staleness of user and DEX states, and expected mis-pricing of states from users. The next section discusses protections against both of these sources of MEV.

==> Structure.tex <==
\section{Deliverable}

\begin{enumerate}
    \item Formalize/propose a categorization/categorization of MEV applicable for explaining cross-domain MEV.
    \item Use the categorizations to explain cross-domain MEV, or where cross-domain MEV fits in within these categorizations. 
    \item Discuss the conflicting cost of certain cross-domain implementations, and the value gained by increases cross-domain expressiveness.
    \item Introduce protections against (cross-domain) MEV. 
        \begin{itemize}
            \item Make a comparison table in this regard.
            \item 
        \end{itemize}
    \item Provide a case study comparison of MDSs and SDSs, sketching the equality of SDS and MDS. 
\end{enumerate}

==> UnityIsStrength.tex <==
\section{Comparing Single Domain Sequencers to an all powerful sequencer}

First, let us assume there is no additional running cost for a single sequencer sequencing multiple domains vs a set of individual sequencers for many domains. 

What does it mean to be a sequencer? For this, we look at what is required in the single sequencer over many domains case. 

Due to the constraints of blockchains with faster block times, the sequencer must be able to commit to an ordering of transactions in the slower blockchains before the block is produced. 

To ensure the network is not spammed and transactions included in the sequencer are executed, block producers are likely required to provide constraints to the sequencer. This particular point is beyond the scope of this analysis. We do however assume that there is a known fee $fee$ which ensures a transaction submitted to the sequencer at time $t$ is included in the sequencer by time $t+\delta$, for some $\delta>0$. In reality, $fee$ is likely to be a function of the number of transactions already sequenced for inclusion, and the time to block production. \textbf{NOTE}: This definition assumes sequencers are censorship resistant. 

The base case for this analysis is the 2-domain scenario. Each sequencer can choose to insert arbitrarily many transactions in their respective sequencers before $t+\delta$. 

From the previous section, we have hypothesized that all MEV is as a result of mis-pricing and mis-timing (much like the frontier atomic vs. signal categorization, although including censorship). As $\delta$ approaches 0, MEV as a result of mis-timing approaches 0. This is analogous to a result from \footnote{\url{https://moallemi.com/ciamac/papers/lvr-fee-model-2023.pdf}}. When the time available to act on a state tends to 0, the expected profit resulting from mis-timing also tends to 0. 

Thus, any viable sequencer, shared or single-domain, with sub-second confirmation times approaches the same limit of approximately 0 MEV as a result of mis-timing. 

The question remains as to whether MEV as a result of mis-pricing varies in the shared sequencer case. To compare the two scenarios, consider a mis-priced transaction applicable to a single domain. 


In the shared sequencer, the sequencer can optimally execute any atomic arbitrage which occurs on either of the domains. Let us say this requires $x$ transactions on the second domain. In the shared sequencer, this is an opportunity cost of approximately $x* fee$. In the single domain case, the sequencer can optimally execute any arbitrage on their own domain. They can also submit orders to be executed in the sequencer of the second domain. This costs $x* fee$. In the single domain case, it might be suggested that the lack of atomicity in the second domain has some risk-associated cost for the sequencer. 

An important question emerging from all of this is what censorship resistance do we have? Can players still be front-run? Is being front-run across 2 domains for 2 transactions worse than being front run on 1-domain for both of those transactions? Let's say there is a searcher with the ability to execute arbitrage across multiple domains. Executing the arb on the shared sequencer makes the arbitrage obvious to the sequencer. Executing the arbitrage across the individual domains makes it less clear. Furthermore, even if a player on one of the domains sees the intent to perform cross-domain arbitrage, these players are not necessarily equipped to perform it. On the contrary, all players in the shared sequencer must be assumed to have the ability to act on the cross-domain arbitrage. 

As such, the MEV in the shared sequencer for a cross-domain atomic(ish) arbitrage is maximal, while the MEV across the individual domains is potentially less than this. Can we argue that the margins on cross-domain arbitrage approaches the limit of the opportunity on the individual legs? In the short- to medium-term as the blockchain space continues to mature. \textbf{Intuition/consensus: yes, Evidence: no}.

There are clear added costs to sequencing multiple domains for an individual domain, placing higher resource constraints on the universe of chains, explicitly centralizing the security of the universe onto one protocol, and forcing chains to conform to a common design to enable compatibility with the shared sequencer. On the other hand, there is a clear benefit to a single shared sequencer for users over a set of (semi-)independent domains (in the single domain case, inter-domain communication is possible, although a TTP is needed \cite{Zamyatin2019Communication}). When users are offered the ability to submit transactions atomically across multiple domains through the shared sequencer, cross-domain interactions become more expressive. Importantly, the current promise of sequencers is just for ordering, and not for execution. This guarantee is relatively weak. 

Can this functionality be replicated in the single-domain sequencer model? For an inclusion delay $\delta$ on both the shared sequencer and single domain sequencers, all legs can be front-run in both the shared and single-domain case. As such, having a shared sequencer offers no benefit.  

